From Reflection to Perfection: Scaling Inference-Time Optimization for Text-to-Image Diffusion Models via Reflection Tuning

Recent text-to-image diffusion models achieve impressive visual quality through extensive scaling of training data and model parameters, yet they often struggle with complex scenes and fine-grained details. Inspired by the self-reflection capabilities emergent in large language models, we propose ReflectionFlow, an inference-time framework enabling diffusion models to iteratively reflect upon and refine their outputs. ReflectionFlow introduces three complementary inference-time scaling axes: (1) noise-level scaling to optimize latent initialization; (2) prompt-level scaling for precise semantic guidance; and most notably, (3) reflection-level scaling, which explicitly provides actionable reflections to iteratively assess and correct previous generations. To facilitate reflection-level scaling, we construct GenRef, a large-scale dataset comprising 1 million triplets, each containing a reflection, a flawed image, and an enhanced image. Leveraging this dataset, we efficiently perform reflection tuning on state-of-the-art diffusion transformer, FLUX.1-dev, by jointly modeling multimodal inputs within a unified framework. Experimental results show that ReflectionFlow significantly outperforms naive noise-level scaling methods, offering a scalable and compute-efficient solution toward higher-quality image synthesis on challenging tasks.

==> Tabletex/Potential.tex <==
\begin{table}[t] % 使用 table 而不是 table*，以适应单栏
% \vspace{-4mm}
\centering
% \vspace{-3mm}
% \fontsize{8pt}{10pt}\selectfont
\resizebox{\columnwidth}{!}{ % 调整为单栏宽度
\begin{tabular}{@{}c >{\centering\arraybackslash}p{4cm} | c c c@{}} % 保留所需的四列
\toprule
 & \textbf{Methods}  & \textbf{Overall} & \textbf{Colors} & \textbf{Position} \\
\cmidrule{1-5}
& Noise Scaling &  0.87  &  0.93 & 0.45 \\
& Noise \& Prompt Scaling & 0.91  & 0.94  & 0.75 \\
& \model  & \textbf{0.96}  &  \textbf{0.99} & \textbf{0.94} \\
\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{Oracle verifier results across various scaling dimensions.}
\label{tab:potential}
\vspace{-3mm}
\end{table}

